Modern Evolution Strategies for Creativity: Fitting Concrete Images and Abstract Concepts

Evolutionary algorithms have been used in the digital art scene since the 1970s. A popular application of genetic algorithms is to optimize the procedural placement of vector graphic primitives to resemble a given painting. In recent years, deep learning-based approaches have also been proposed to generate procedural drawings, which can be optimized using gradient descent. In this work, we revisit the use of evolutionary algorithms for computational creativity. We find that modern evolution strategies (ES) algorithms, when tasked with the placement of shapes, offer large improvements in both quality and efficiency compared to traditional genetic algorithms, and even comparable to gradient-based methods. We demonstrate that ES is also well suited at optimizing the placement of shapes to fit the CLIP model, and can produce diverse, distinct geometric abstractions that are aligned with human interpretation of language. Videos and demo: https://es-clip.github.io/

==> figures/es-basic-mona-lisa.tex <==
\begin{figure}[!htb]

\captionsetup[subfigure]{labelformat=empty}
\centering

\begin{subfigure}[t]{0.20\textwidth}
    \centering
    \includegraphics[width=\textwidth]{es-basic-target.png}
    \caption{``Mona Lisa''}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.20\textwidth}
    \centering
    \includegraphics[width=\textwidth]{es-basic-evolved-results.png}
    \caption{Evolved Results}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.54\textwidth}
    \centering
    \includegraphics[width=\textwidth]{es-basic-evolution-process.gif-coalesce-3x8.png}
    \caption{Evolution Process}
\end{subfigure}
\caption{
The simple genetic algorithm proposed in \citep{alteredqualia2008evolutiongenetic} fits 50 triangles to visually approximate Mona Lisa. Here, the algorithm runs for 10,000 steps, resulting in $90\%$ fitness.}
\label{fig:es-basic-mona-lisa}
\end{figure}


==> figures/es-clip-two-runs-examples.tex <==
\begin{figure}[!htb]

\captionsetup[subfigure]{labelformat=empty}
\centering


\begin{subfigure}[h]{0.6\textwidth}
\newcommand{\imgwidth}{2.3cm}
\centering
\begin{tabular}{ccc}
    \toprule
    \textbf{Target Image} & \textbf{50 Triangles} & \textbf{200 Triangles} \\
    \midrule
    \includegraphics[width=\imgwidth]{es-ours-darwin-target.jpg} &
        \includegraphics[width=\imgwidth]{es-ours-darwin-50-triangles-evolution-process.gif-coalesce-1x1.png} &
        \includegraphics[width=\imgwidth]{es-ours-darwin-200-triangles-evolution-process.gif-coalesce-1x1.png} \\
    ``Darwin'' & Fitness = $99.1\%$ & Fitness = $99.5\%$ \\
    \midrule
    \includegraphics[width=\imgwidth]{es-ours-johnkoza-target.jpg} &
        \includegraphics[width=\imgwidth]{es-ours-johnkoza-50-triangles-evolution-process.gif-coalesce-1x1.png} &
        \includegraphics[width=\imgwidth]{es-ours-johnkoza-200-triangles-evolution-process.gif-coalesce-1x1.png} \\
    ``John Koza'' & Fitness = $99.2\%$ & Fitness = $99.5\%$ \\
    \midrule
    \includegraphics[width=\imgwidth]{es-ours-monalisa-target.jpg} &
        \includegraphics[width=\imgwidth]{es-ours-monalisa-50-triangles-evolution-process.gif-coalesce-1x1.png} &
        \includegraphics[width=\imgwidth]{es-ours-monalisa-200-triangles-evolution-process.gif-coalesce-1x1.png} \\
    ``Mona Lisa'' & Fitness = $99.4\%$ & Fitness = $99.7\%$ \\
    \bottomrule
\end{tabular}
\end{subfigure}
\begin{subfigure}[h]{0.38\textwidth}
\newcommand{\imgwidth}{5.575cm}
\centering
\begin{tabular}{p{\imgwidth}}
    \toprule
    \includegraphics[width=\imgwidth]{es-ours-darwin-50-triangles-evolution-process.gif-coalesce-4x5.png} \\
    \midrule
    \includegraphics[width=\imgwidth]{es-ours-darwin-200-triangles-evolution-process.gif-coalesce-4x5.png} \\
    \bottomrule
\end{tabular}
\end{subfigure}

\caption{On the left, qualitative and quantitative results two runs of ES with CLIP.
On the right, the details of evolution process when fitting target image ``A drawing of a cat''.
}
\label{fig:es-ours-two-runs-examples}
\end{figure}

==> figures/es-clip-two-runs.tex <==
\begin{figure}[!htb]

\captionsetup[subfigure]{labelformat=empty}
\centering


\begin{subfigure}[h]{1.0\textwidth}
\newcommand{\imgwidth}{2.4cm}
    \centering
    \begin{longtable}{ccc}
    \toprule
    \textbf{Target Text} & \textbf{Run 1} & \textbf{Run 2} \\
    
    \midrule
    
    \textbf{``Landscape''} &
        \includegraphics[width=\imgwidth]{es-clip-Landscape-run-1.gif-coalesce-1x1.png} &
        \includegraphics[width=\imgwidth]{es-clip-Landscape-run-2.gif-coalesce-1x1.png} \\
    
    \midrule
    
    \textbf{``Human''} &
        \includegraphics[width=\imgwidth]{es-clip-Human-run-1.gif-coalesce-1x1.png} &
        \includegraphics[width=\imgwidth]{es-clip-Human-run-2.gif-coalesce-1x1.png} \\
    
    \midrule
    
    \textbf{``Self''} &
        \includegraphics[width=\imgwidth]{es-clip-Self-run-1.gif-coalesce-1x1.png} &
        \includegraphics[width=\imgwidth]{es-clip-Self-run-2.gif-coalesce-1x1.png} \\
    
    \midrule
    
    \textbf{``Family vacation to Walt Disney World''} &
        \includegraphics[width=\imgwidth]{es-clip-Family_vacation_to_Walt_Disney_World-run-1.gif-coalesce-1x1.png} &
        \includegraphics[width=\imgwidth]{es-clip-Family_vacation_to_Walt_Disney_World-run-2.gif-coalesce-1x1.png} \\
    
    \midrule
    
    \textbf{``A painting of a sunset''} &
        \includegraphics[width=\imgwidth]{es-clip-A_painting_of_a_sunset-run-1.gif-coalesce-1x1} &
        \includegraphics[width=\imgwidth]{es-clip-A_painting_of_a_sunset-run-2.gif-coalesce-1x1} \\
    
    \midrule
    
    \textbf{``A spaceship flying in a starry sky''} &
        \includegraphics[width=\imgwidth]{es-clip-A_spaceship_flying_in_a_starry_sky-run-1.gif-coalesce-1x1} &
        \includegraphics[width=\imgwidth]{es-clip-A_spaceship_flying_in_a_starry_sky-run-1.gif-coalesce-1x1} \\
        
    \midrule
    
    \textbf{``A picture of Japan''} &
        \includegraphics[width=\imgwidth]{es-clip-A_picture_of_Japan-run-1.gif-coalesce-1x1} &
        \includegraphics[width=\imgwidth]{es-clip-A_picture_of_Japan-run-2.gif-coalesce-1x1} \\
    
    \bottomrule
    
    \end{longtable}

\end{subfigure}

\caption{Fitting triangles to text using CLIP. Most of the text example are from CLIPDraw.}
\label{fig:es-clip-two-runs}
\end{figure}
